Focusing on Refinement Typing

We present a logically principled foundation for systematizing, in a way that works with any computational effect and evaluation order, SMT constraint generation seen in refinement type systems for functional programming languages. By carefully combining a focalized variant of call-by-push-value, bidirectional typing, and our novel technique of value-determined indexes, our system generates solvable SMT constraints without existential (unification) variables. We design a polarized subtyping relation allowing us to prove our logically focused typing algorithm is sound, complete, and decidable. We prove type soundness of our declarative system with respect to an elementary domain-theoretic denotational semantics. Type soundness implies, relatively simply, the total correctness and logical consistency of our system. The relative ease with which we obtain both algorithmic and semantic results ultimately stems from the proof-theoretic technique of focalization.

==> ex-list.tex <==
Let $P$ be a positive type
that is well-formed under empty $\Theta$ and $\Xi$,
i.e. such that $\judgetp{}{P}{\cdot}$.
Let $F = I \oplus \Const{P} \otimes \Id \otimes I$.
The initial $F$-algebra $\mu F$ is (finite, but arbitrarily long)
lists of elements of type $P$.
Say we want to refine $\mu F$ to lists of $n$ elements
(where $n \geq 0$ is fixed), i.e. we want to form the refinement type
$\comprehend{\nu : \mu F}{\textsf{length}\,{\nu} = n}$.
In our system, we obtain the function \textsf{length} by providing a suitable
algebra $\judgealgebra{\cdot}{\cdot}{\alpha}{F}{\kindnat}$
such that the universal property of initial algebras
yields the unique function $\Fold{F}{\alpha} = \textsf{length} : \mu F \to \kindnat$.
To this end, put
\[
  \alpha = \inl \clause{\unitexp}{0}
    \matchor \inr \clause{(\wild, (a, \unitexp))}{1 + a}
    \matchor \cdot
\]

We will now demonstrate how to unroll the refinement type 
$\comprehend{\nu : \mu F}{\Fold{F}{\alpha}\,{\nu} =_\kindnat n}$
using the rules of \Figureref{fig:unroll}.
Starting with \Figureref{fig:declwf-type},
it's easy to check that
\[
  \judgetp{}{\comprehend{\nu : \mu F}{\Fold{F}{\alpha}\,{\nu} =_\kindnat n}}{\cdot}
\]
Further, using \Figureref{fig:auxpat}, we have
\[
  \composeinj{1}{\alpha}{\clause{\unitexp}{0}}
\]
and
\[
  \composeinj{2}{\alpha}{\clause{(\wild, (a, \unitexp))}{1+a}}
\]
Now, let $\mathcal{D}_1$ be the following derivation:
\[
  \Infer{\DeclUnrollUnit}
  {}
  {
    \judgeunroll{\cdot}{\cdot}{\nu:I[\mu F]}{(\clause{\unitexp}{0})}{I\;\Fold{F}{\alpha}\,{\nu}}{n}
      {1 \land n = 0}{\kindnat}
  }
\]
Next, let $\mathcal{D}_2$ be the following derivation:
\[\scalebox{0.9}{$
    \Infer{\DeclUnrollConst}
    {
        \Infer{\DeclUnrollId}
        {
          \Infer{\DeclUnrollUnit}
          {}
          {
            \judgeunroll{a:\kindnat}{a:\kindnat}
              {\nu: I[\mu F]}
              {(\clause{\unitexp}{1+a})}
              {I\;\Fold{F}{\alpha}\;\nu}
              {n}
              {1 \land n = 1 + a}
              {\kindnat}
          }
        }
      {
        \judgeunroll*{\cdot}{\cdot}
          {\nu:(\Id \otimes I)[\mu F]}
          {(\clause{(a, \unitexp)}{1+a})}
          {(\Id\otimes I)\;\Fold{F}{\alpha}\;\nu}
          {n}
          {\extype{a:\kindnat}
             {\comprehend{\nu:\mu F}{\Fold{F}{\alpha}\,{\nu} =_\kindnat a}
                              \times (1 \land n = 1 + a)}}
          {\kindnat}
      }
    }
  {
    \judgeunroll*{\cdot}{\cdot}
      {\nu:(\Const{P}\otimes\Id \otimes I)[\mu F]}
      {(\clause{(\wild, (a, \unitexp))}{1+a})}
      {(\Const{P}\otimes\Id \otimes I)\;\Fold{F}{\alpha}\,{\nu}}
      {n}
      {P \times \extype{a:\kindnat}
        {\comprehend{\nu:\mu F}{\Fold{F}{\alpha}\,{\nu} =_\kindnat a}
                           \times (1 \land n = 1 + a)}}
      {\kindnat}
  }
$}\]
Putting all this together, we derive:
\[
  \Infer{\DeclUnrollSum}
  {
    \arrayenvb{\vdots \\ \composeinj{1}{\alpha}{\clause{\unitexp}{0}}}
    \\
    \arrayenvb{\vdots \\ \composeinj{2}{\alpha}{\clause{(\wild, (a, \unitexp))}{1+a}}}
    \\
    \mathcal{D}_1
    \\
    \mathcal{D}_2
  }
  {
    \judgeunroll*{\cdot}{\cdot}
    {\nu:(I \oplus \Const{P} \otimes \Id \otimes I)[\mu F]}
    {\alpha}
    {(I \oplus \Const{P} \otimes \Id \otimes I)\;\Fold{F}{\alpha}\,{\nu}}
    {n}
    {(1 \land n = 0) + P \times \extype{a:\kindnat}
      {\comprehend{\nu:\mu F}{\Fold{F}{\alpha}\,{\nu} =_\kindnat a}
                         \times (1 \land n = 1 + a)}}
    {\kindnat}
  }
\]

%
%
%


==> fig-algtyping-old.tex <==
\begin{figure}[htbp]
  \centering

  \judgbox{\algsub[\pm]{\Theta}{A}{B}{\Wah}{\Theta'}}
      {
        Under input context $\Theta$, type $A$ is a $\pm$-polar subtype of $B$,\\
        with output Wahnsinnsshow $\Wah$ and output context $\Theta'$
      }

\begin{mathpar}
  \Infer{\AlgSubPosVoid}
        { }
        {
          \algsub[+]{\Theta}{0}{0}{\True}{\Theta}
        }
  \and
  \Infer{\AlgSubPosUnit}
        { }
        {\algsub[+]{\Theta}{1}{1}{\True}{\Theta}}
  \and
  \Infer{\AlgSubPosProd}
        {
          \algsub[+]{\Theta}{P_1}{Q_1}{\Wah_1}{\Theta_1}
          \\
          \algsub[+]{\Theta_1}{[\Theta_1]P_2}{[\Theta_1]Q_2}{\Wah_2}{\Theta_2}
       }
        {
          \algsub[+]{\Theta}{P_1 \times P_2}{Q_1 \times Q_2}{[\Theta_2]\Wah_1 \land \Wah_2}{\Theta_2}
        }
  \and
  \Infer{\AlgSubPosSum}
        {
          \algsub[+]{\Theta}{P_1}{Q_1}{\Wah_1}{\Theta_1}
          \\
          \algsub[+]{\Theta_1}{[\Theta_1]P_2}{[\Theta_1]Q_2}{\Wah_2}{\Theta_2}
       }
        {
          \algsub[+]{\Theta}{P_1 + P_2}{Q_1 + Q_2}{[\Theta_2]\Wah_1 \land \Wah_2}{\Theta_2}
        }
  \and
  \Infer{\AlgSubPosWithL}
        {
          \algsub[+]{\Theta, \phi}{P}{Q}{\Wah}{\Theta'}
        }
        {
          %
          \algsub[+]{\Theta}{P \andty \phi}{Q}{\phi \implies \Wah}{\Theta'}
        }
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  \and
  \Infer{\AlgSubPosWithR}
        {
          \algsub[+]{\Theta}{P}{Q}{\Wah}{\Theta'}
        }
        {
          \algsub[+]{\Theta}{P}{Q \land \phi}{\Wah \land [\Theta']\phi}{\Theta'}
        }
  \and
  \Infer{\AlgSubPosExL}
        {
          \algsub[+]{\Theta, a:\tau}{P}{Q}{\Wah}{\Theta', a:\tau, \Theta''}
        }
        {
          \algsub[+]{\Theta}{\extype{a:\tau} P}{Q}
              {\forall a:\tau.\Wah}
              {\Theta'}
        }
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  \and 
  \Infer{\AlgSubPosExR}
        { 
          \algsub[+]{\Theta, \ahat:\tau}{P}{[\ahat/a] Q}{\Wah}{\Theta', \hypeq{\ahat}{\tau}{t}, \Phi}
          \\
          P \text{~not $\exists$ or $\andty$}
        }
        {
          \algsub[+]{\Theta}{P}{\extype{a:\tau} Q}{\Wah}{\Theta', \Phi}
        }
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  \and
  \Infer{\AlgSubPosFix}
        {
          \ground{\comprehend{\nu:\mu F}{\Fold{F}{\alpha}\,\nu =_\tau t}}
          \\
          \alltype{\ahat \in \dom{\Theta}}{[\Theta]t' \neq \ahat}
        }
        {
          \algsub[+]
             {\Theta}
             {\comprehend{\nu:\mu F}{\Fold{F}{\alpha}\,\nu =_\tau t}}
             {\comprehend{\nu:\mu F}{\Fold{F}{\alpha}\,\nu =_\tau t'}}
             {t = [\Theta]t'}
             {\Theta}
        }
  \and
  \Infer{\AlgSubPosFixInst}
        {
          \ground{\comprehend{\nu:\mu F}{\Fold{F}{\alpha}\,\nu =_\tau t}}
          \\
          \judgeterm{\Theta_1}{t}{\tau}
        }
        {
          \algsub[+]
             {\Theta_1, \ahat:\tau, \Theta_2}
             {\comprehend{\nu:\mu F}{\Fold{F}{\alpha}\,\nu =_\tau t}}
             {\comprehend{\nu:\mu F}{\Fold{F}{\alpha}\,\nu =_\tau \ahat}}
             {
               %
               t = t
             }
             {\Theta_1, \hypeq{\ahat}{\tau}{t}, \Theta_2}
        }
  \and
  \Infer{\AlgSubPosFixInstFun}
        {
          \ground{\comprehend{\nu:\mu F}{\Fold{F}{\alpha}\,\nu =_\tau t}}
          \\
          n > 0
          \\
          \alltype{k \in \{1, \dots, n\}} (\ahat_k:\tau_k) \in \Theta
          \\
          \alltype{k \in \{1, \dots, n\}} \judgeterm{\Theta}{t_k}{\tau_k}
          \\
          \ahat_1, \dots, \ahat_n \in \fev{F'}
          \\
          \rho = t_1/\ahat_1, \dots, t_n/\ahat_n
          \\
          [\rho]F' = F
          \\
          \algsub[+]
          {\Theta}
          {\comprehend{\nu:\mu F}{\Fold{F}{\alpha}\,\nu =_\tau t}}
          {[\rho]\comprehend{\nu:\mu F'}{\Fold{F'}{\alpha}\,\nu =_\tau t'}}
          {\Wah}
          {\Theta'}
        }
        {
          \algsub[+]
             {\Theta}
             {\comprehend{\nu:\mu F}{\Fold{F}{\alpha}\,\nu =_\tau t}}
             {\comprehend{\nu:\mu F'}{\Fold{F'}{\alpha}\,\nu =_\tau t'}}
             {\Wah}
             {\inst{\rho}{\Theta'}}
        }
  \\
  \Infer{\AlgSubPosDownshift}
        {
        %
        %
        %
        }
        {
          \algsub[+]{\Theta}{\downshift{N}}{\downshift{M}}{\negsubprob{N}{M}}{\Theta}
        }
  \and
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  \Infer{\AlgSubNegUpshift}
        {
        }
        {
          \algsub[-]{\Theta}{\upshift{P}}{\upshift{Q}}
          {\possubprob{P}{Q}}{\Theta}
        }
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  \and
  \Infer{\AlgSubNegImpL}
        {
          \algsub[-]{\Theta}{N}{M}{\Wah}{\Theta'}
          %
          %
        }
        {
          \algsub[-]{\Theta}{\phi \implies N}{M}
            {\Wah \land [\Theta']\phi}{\Theta'}
        }
  \and
  \Infer{\AlgSubNegImpR}
        {\algsub[-]{\Theta, \phi}{N}{M}{\Wah}{\Theta'} }
        %
        {\algsub[-]{\Theta}{N}{\phi \implies M}{\phi\implies\Wah}{\Theta'} }
  \and
  %
  %
  %
  %
  %
  %
  %
  %
  \Infer{\AlgSubNegAllL}
        {
          \algsub[-]{\Theta,\ahat:\tau}{[\ahat/a]N}{M}{\Wah}{\Theta', \hypeq{\ahat}{\tau}{t}, \Phi}
          \\
          M \text{~not $\forall$ or $\implies$}
        }
        {\algsub[-]{\Theta}{\alltype{a:\tau} N}{M}{\Wah}{\Theta', \Phi} }
  \and
  \Infer{\AlgSubNegAllR}
        {\algsub[-]{\Theta, a:\tau}{N}{M}{\Wah}{\Theta', a:\tau, \Theta''} }
        {
          \algsub[-]{\Theta}{N}{\alltype{a:\tau} M}{\alltype{a:\tau} \Wah}{\Theta'}
        }
  \and
  \Infer{\AlgSubNegArrow}
        {
          \algsub[+]{\Theta}{Q}{P}{\Wah_1}{\Theta_1}
          \\
          \algsub[-]{\Theta_1}{[\Theta_1]N}{[\Theta_1]M}{\Wah_2}{\Theta_2}
        }
        {
          \algsub[-]{\Theta}{P -> N}{Q -> M}
            {[\Theta_2]\Wah_1 \land \Wah_2}{\Theta_2}
        } 
\end{mathpar}

  \caption{Algorithmic subtyping}
  \label{fig:algsubtyping}
\end{figure}


\begin{figure}[htbp]
  \centering

  \judgbox{\algsynhead{\Theta}{\Gamma}{h}{P}{\Theta'}}
      {Under input contexts $\Theta$ and $\Gamma$,
        head $h$ synthesizes $P$,
        with output context $\Theta'$}

      \begin{mathpar}
        \Infer{}
          {
            (x : P) \in \Gamma
          }
          {
            \algsynhead{\Theta}{\Gamma}{x}{P}{\Theta}
          }
        \and
        \Infer{}
          {
            \judgetp{\Theta}{P}{\Xi}
            \\
            %
            \algchk{\Theta}{\Gamma}{v}{P}{\chi}{\Theta'}
            \\
            \algneg{\Theta'}{\Gamma}{\chi}
          }
          {
            \algsynhead{\Theta}{\Gamma}{\annoexp{v}{P}}{P}{\Theta'}
          }
      \end{mathpar}


  \judgbox{\algsynexp{\Theta}{\Gamma}{\be}{N}{\Theta'}}
      {Under input contexts $\Theta$ and $\Gamma$,
        bound expression $\be$ synthesizes $N$,\\
        with output context $\Theta'$}

      \begin{mathpar}
        %
        \Infer{}
          { 
            \arrayenvb{
              \algsynhead{\Theta}{\Gamma}{h}{Q}{\Theta''} \\
              \judgeleadsto{\Theta}{Q}{\downshift{N}}{\Phi}
            }
            \\
            \arrayenvb{
              \algspine{\Theta''}{\Gamma}{s}{N}{\upshift{P}}{\chi}{\Theta'} \\
              \algneg{\Theta'}{\Gamma}{\chi}
            }
          }
          { \algsynexp{\Theta}{\Gamma}{h(s)}{\upshift{P}}{\Theta'} }
        \and
        %
        \Infer{}
          {
            \judgetp{\Theta}{P}{\Xi}
            \\
            \algchkneg{\Theta}{\Gamma}{e}{\upshift{P}}
          }
          { \algsynexp{\Theta}{\Gamma}{\annoexp{e}{\upshift{P}}}{\upshift{P}}{\Theta} }
      \end{mathpar}


  \judgbox{\algchk{\Theta}{\Gamma}{v}{P}{\chi}{\Theta'}}
        {Under inputs contexts $\Theta$ and $\Gamma$,
          the value $v$ checks against type $P$,\\
          with output computation problems $\chi$ and output context $\Theta'$}
  
      \begin{mathpar}
        \Infer{}
            {(x:Q)\in\Gamma \\ \algsub[+]{\Theta}{Q}{P}{\Wah}{\Theta'}}
            {
              \algchk{\Theta}{\Gamma}{x}{P}{\Wah}{\Theta'}
            }
        \\
        \Infer{}
            {
            }
            {
              \algchk{\Theta}{\Gamma}{\unit}{\unitty}{\cdot}{\Theta}
            }
        \and
        \Infer{}
            {
              \algchk{\Theta}{\Gamma}{v_1}{P_1}{\chi_1}{\Theta''}
              \\
              \algchk{\Theta''}{\Gamma}{v_2}{[\Theta'']P_2}{\chi_2}{\Theta'}
            }
            {
              \algchk{\Theta}{\Gamma}{\pair{v_1}{v_2}}
                {(P_1 \times P_2)}{[\Theta']\chi_1, \chi_2}{\Theta'}
            }
        \and
        \Infer{}
            {
              \algchk{\Theta}{\Gamma}{v_k}{P_k}{\chi}{\Theta'}
            }
            {
              \algchk{\Theta}{\Gamma}{\inj{k}{v_k}}{(P_1 + P_2)}{\chi}{\Theta'}
            }
        \and
        \Infer{}
            {
              %
              \judgeunroll{\cdot}{\Theta}{\nu:F[\mu F]}{\alpha}{F\; \Fold{F}{\alpha}\;\nu}{t}{P}{\tau}
              \\
              \algchk{\Theta}{\Gamma}{v}{P}{\chi}{\Theta'}
            }
            {
              \algchk{\Theta}{\Gamma}{\into{v}}
                {\comprehend{\nu : \mu F}{\Fold{F}{\alpha}\,{\nu} =_\tau t}}{\chi}{\Theta'}
            }
        \and
        \Infer{}
            {
            }
            {
              \algchk{\Theta}{\Gamma}{\thunk{e}}{\downshift{N}}{(e <= N)}{\Theta}
            }
        \and
        \Infer{}
            {
              \algchk{\Theta, \ahat:\tau}{\Gamma}{v}{[\ahat / a]P}{\chi}{\Theta', \hypeq{\ahat}{\tau}{t}}
              %
            }
            {
              \algchk{\Theta}{\Gamma}{v}{(\extype{a : \tau} P)}{\chi}{\Theta'}
            }
        \and
        \Infer{}
            {
              \algchk{\Theta}{\Gamma}{v}{P}{\chi}{\Theta''}
              \\
              \alginst{\Theta''}{\phi}{\Theta'}
            }
            {
              \algchk{\Theta}{\Gamma}{v}{(P \andty \phi)}
                {([\Theta']\phi, [\Theta']\chi)}{\Theta'}
            }
        %
        %
        %
        %
        %
        %
        %
        %
        %
      \end{mathpar}


  \judgbox{\algchkneg{\Theta}{\Gamma}{e}{N}}
          {
            Under input contexts $\Theta$ and $\Gamma$,
            expression $e$ checks against $N$
          }
  \begin{mathpar}
    %
    \Infer{}
          { 
            %
            \algchk{\Theta}{\Gamma}{v}{P}{\chi}{\Theta'} 
            \\
            \algneg{\Theta'}{\Gamma}{\chi}
          }
          {
            \algchkneg{\Theta}{\Gamma}{\Return{v}}{\upshift{P}} 
          }
    \and 
    %
    \Infer{}
          { \algsynexp{\Theta}{\Gamma}{\be}{\upshift{P}}{\Theta'} \\
            \algchkneg{\Theta'}{\Gamma, x:P}{e}{N} }
          { \algchkneg{\Theta}{\Gamma}{\Let{x}{\be}{e}}{N} }
    \and
    %
    \Infer{}
          {
            \algsynhead{\Theta}{\Gamma}{h}{P}{\Theta'}
            \\
            %
            \judgechkmatch{\Theta'}{\Gamma}{P}{\clauses{\pa}{e}{i}{I}}{N}
          }
          {
            \algchkneg{\Theta}{\Gamma}{\match{h}{\clauses{\pa}{e}{i}{I}}}{N}
          }
    \and 
    %
    \Infer{}
          { \algchkneg{\Theta}{\Gamma, x:P}{e}{N} }
          { \algchkneg{\Theta}{\Gamma}{\fun{x}{e}}{P \to N} }
    \and
    %
    \Infer{}
    {
      \judgechkexp{\Theta}{\Gamma, f:\downshift{N}}{e}{N}
      \\
      (f\text{ is well-founded})
    }
    { \judgechkexp{\Theta}{\Gamma}{\rec{f}{e}}{N} }
    \and
    %
    \Infer{}
          { \algchkneg{\Theta, \phi}{\Gamma}{e}{N} \\ \Intro{e} }
          { \algchkneg{\Theta}{\Gamma}{e}{\phi \implies N} }
    \and
    %
    \Infer{}
          { \algchkneg{\Theta, a:\tau}{\Gamma}{e}{N} \\ \Intro{e} }
          { \algchkneg{\Theta}{\Gamma}{e}{(\alltype{a:\tau} N)} }
  \end{mathpar}

  \caption{Algorithmic typing stuff (2)}
  \label{fig:algtyping-more}
\end{figure}



\begin{figure}[htbp]
  \centering
\judgbox{\judgechkmatch{\Theta}{\Gamma}{P}{\clauses{\pa}{e}{i}{I}}{N}}
        {Under $\Theta$ and $\Gamma$, each pattern $r_i$ is of type $P$ \\
          and has a branch expression $e_i$ that checks against type $N$}
\begin{mathpar}
  \Infer{\DeclChkMatchEx}
        {\judgechkmatch{\Theta, a:\tau}{\Gamma}{P}{\clauses{\pa}{e}{i}{I}}{N}}
        {\judgechkmatch{\Theta}{\Gamma}{\extype{a:\tau}{P}}{\clauses{\pa}{e}{i}{I}}{N}}
  \and
  \Infer{\DeclChkMatchWith}
        {\judgechkmatch{\Theta, \phi}{\Gamma}{P}{\clauses{\pa}{e}{i}{I}}{N}}
        {\judgechkmatch{\Theta}{\Gamma}{P \land \phi}{\clauses{\pa}{e}{i}{I}}{N}}
  \and
  \Infer{\DeclChkMatchUnit}
        { \judgechkexp{\Theta}{\Gamma}{e}{N} }
        { \judgechkmatch{\Theta}{\Gamma}{1}{\setof{\clause{\unit}{e}}}{N} }
  \and
  \Infer{\DeclChkMatchPair}
        { \judgechkexp{\Theta}{\Gamma, x_2:P_2, x_1:P_1}{e}{N} }
        {
          \judgechkmatch{\Theta}{\Gamma}{P_1 \times P_2}
          {\setof{\clause{\pair{x_1}{x_2}}{e}}}{N}
        }
  \and
  \Infer{\DeclChkMatchSum}
        { \judgechkexp{\Theta}{\Gamma, x_1:P_1}{e_1}{N} \\
          \judgechkexp{\Theta}{\Gamma, x_2:P_2}{e_2}{N} }
        { \judgechkmatch{\Theta}{\Gamma}{P_1 + P_2}{\setof{ \clause{\inl{x_1}}{e_1} \bnfalt \clause{\inr{x_2}}{e_2}}}{N} }
  \and
  \Infer{\DeclChkMatchVoid}
        { }
        { \judgechkmatch{\Theta}{\Gamma}{0}{\setof{}}{N} }
  \and
  \Infer{\DeclChkMatchFix}
        {
          \judgeunroll{\cdot}{\Theta}{\nu:F[\mu F]}{\alpha}{F\;\Fold{F}{\alpha}\;\nu}{t}{P}{\tau}
          \\
          \judgechkexp{\Theta}{\Gamma, x:P}{e}{N}
        }
        {
          \judgechkmatch{\Theta}{\Gamma}{\comprehend{\nu:\mu F}
            {\Fold{F}{\alpha}\,{\nu} =_\tau t}}{\setof{\clause{\roll{x}}{e}}}{N}
        }
\end{mathpar}


  \judgbox{\algspine{\Theta}{\Gamma}{s}{N}{M}{\chi}{\Theta'}}
        {
          Under input contexts $\Theta$ and $\Gamma$,
          passing spine $s$ to a function of type $\downshift{N}$\\
          synthesizes type $M$,
          with output problems $\chi$ and output context $\Theta'$
        }
  \begin{mathpar}
    %
    %
    %
    %
    %
    %
    %
    \Infer{}
        {
          \algspine{\Theta, \ahat : \tau}{\Gamma}{s}{[\ahat/a]{N}}{M}{\chi}{\Theta', \hypeq{\ahat}{\tau}{t}}
        }
        {
          \algspine{\Theta}{\Gamma}{s}{(\alltype{a:\tau}N)}{M}{\chi}{\Theta'}
        }
   \\
   \Infer{}
        {
          \algspine{\Theta}{\Gamma}{s}{N}{M}{\chi}{\Theta'}
        }
        {\algspine{\Theta}{\Gamma}{s}{\phi \implies N}{M}{[\Theta']\phi,\chi}{\Theta'}}
    \and
    \Infer{}
        {
          %
          %
          %
          %
          \algchk{\Theta}{\Gamma}{v}{P}{\chi}{\Theta''}
          \\
          \algspine{\Theta''}{\Gamma}{s}{[\Theta'']N}{M}{\chi'}{\Theta'}
        }
        {\algspine{\Theta}{\Gamma}{v, s}{P -> N}{M}{[\Theta']\chi, \chi'}{\Theta'}}
    \and
    \Infer{}
        {}
        {\algspine{\Theta}{\Gamma}{\cdot}{\upshift{P}}{\upshift{P}}{\True}{\Theta}}
  \end{mathpar}
 
  %
  %
  %
  %
  %

  \judgbox{\alginst{\Theta}{\phi}{\Theta'}}{Proposition $\phi$ instantiates $\Theta$ to $\Theta'$}
  \begin{mathpar}
    \Infer{}
    {
      \ground{t}
    }
    {
      \alginst{\Theta_1, \ahat:\tau, \Theta_2}{\ahat = t}{\Theta_1, \hypeq{\ahat}{\tau}{t}, \Theta_2}
    }
    \Infer{}
    {
      \phi \text{ not of form } \ahat = t \text{ where } \ground{t}
    }
    {
      \alginst{\Theta}{\phi}{\Theta}
    }
  \end{mathpar}

  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %
  %

  \judgbox{\algneg{\Theta}{\Gamma}{\chi}}
          {
            Under input contexts $\Theta$ and $\Gamma$,
            check computation problems $\chi$
          }
  \begin{mathpar}
    \Infer{}
        {
        }
        {
          \algneg{\Theta}{\Gamma}{\cdot}
        }
    \and
    \Infer{}
        {
          \algchkneg{\Theta}{\Gamma}{e}{N}
          \\
          \algneg{\Theta}{\Gamma}{\chi}
        }
        {
          \algneg{\Theta}{\Gamma}{(e <= N), \chi}
        }
    \and
    \Infer{}
        {
          \entailwah{\Theta}{W}
          \\
          \algneg{\Theta}{\Gamma}{\chi}
        }
        {
          \algneg{\Theta}{\Gamma}{W, \chi}
        }
  \end{mathpar}

  \caption{Algorithmic typing stuff (1)}
  \label{fig:algtyping}
\end{figure}

\begin{figure}[htbp]
  \judgbox{\entailwah{\Theta}{\Wah}}{Under $\Theta$, problem $\Wah$ holds}
  \begin{mathpar}
    \Infer{\WTrueProp}
    {
      \judgeentail{\Theta}{\phi}
    }
    {
      \entailwah{\Theta}{\phi}
    }
    \and
    \Infer{\WTrueAnd}
    {
      \entailwah{\Theta}{\Wah_1}
      \\
      \entailwah{\Theta}{\Wah_2}
    }
    {
      \entailwah{\Theta}{\Wah_1 \land \Wah_2}
    }
    \and
    \Infer{\WTrueImpl}
    {
      \entailwah{\Theta, \phi}{\Wah}
    }
    {
      \entailwah{\Theta}{\phi \implies \Wah}
    }
    \and
    \Infer{\WTrueAll}
    {
      \entailwah{\Theta,a:\tau}{\Wah}
    }
    {
      \entailwah{\Theta}{\alltype{a:\tau}\Wah}
    }
    \and
    \Infer{\WTruePosSub}
    {
      \algsub[+]{\Theta}{P}{Q}{\Wah}{\Theta'}
      \\
      \entailwah{\Theta}{\Wah}
    }
    {
      \entailwah{\Theta}{\possubprob{P}{Q}}
    }
    \and
    \Infer{\WTrueNegSub}
    {
      \algsub[-]{\Theta}{N}{M}{\Wah}{\Theta'}
      \\
      \entailwah{\Theta}{\Wah}
    }
    {
      \entailwah{\Theta}{\possubprob{N}{M}}
    }
  \end{mathpar}

  \caption{Constraint verification}
  \label{fig:entail-wah}
\end{figure}

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%

%
%
%
%
%
%
%
%
%


%
%
%


==> fig-denotation-intrinsic.tex <==
\begin{figure}[htbp]

  \begin{grammar}
    Semantic substitutions &
    $\delta$ & \bnfas & $\cdot \bnfalt \delta, d/a \bnfalt \delta, d/x$
  \end{grammar}

  \judgbox{
    |- \delta : \Theta; \Gamma
  }
  {
    We have that
    $\delta$ is a semantic substitution for variables in $\Theta$ and $\Gamma$
  }
  \begin{mathpar}
    \Infer{\EmptySem}
    {
    }
    {
      |- \cdot : \cdot; \cdot
    }
    \and
    \Infer{\IxSem}
    {
      |- \delta : \Theta; \Gamma
      \and
      d \in \sem{}{\tau}
      \and
      a \notin \dom{\Theta}
    }
    {
      |- \delta, d/a : \Theta, a:\tau; \Gamma
    }
    \and
    \Infer{\PropSem}
    {
      |- \delta : \Theta; \Gamma
      \and
      \sem{\delta}{\phi} = \{\bullet\}
    }
    {
      |- \delta : \Theta, \phi; \Gamma
    }
    \and
    \Infer{\ValSem}
    {
      |- \delta : \Theta; \Gamma
      \and
      d \in \sem{\delta}{P}
      \and
      x \notin \dom{\Gamma}
    }
    {
      |- \delta, d/x : \Theta; \Gamma, x:P
    }
  \end{mathpar}

  \caption{Semantic substitution}
  \label{fig:sem-subs}
\end{figure}

\begin{figure}[htbp]
  \centering

  \begin{align*}
    \sem{}{\judgeterm{\Theta}{t}{\tau}} &: \comprehend{\delta}{|- \delta : \overline{\Theta}} \to \sem{}{\tau} \\ 
    \sem{\delta}{a} &= \delta(a)\\
    \sem{\delta}{n} &= n \\
    \sem{\delta}{t_1+t_2} &= \sem{\delta}{t_1}+\sem{\delta}{t_2} \\
    \sem{\delta}{t_1-t_2} &= \sem{\delta}{t_1}-\sem{\delta}{t_2} \\
    \sem{\delta}{(t_1,t_2)} &= (\sem{\delta}{t_1}, \sem{\delta}{t_2}) \\
    \sem{\delta}{\pi_k\,{t}} &= \pi_k\sem{\delta}{t}
    \\[2em]
    \sem{}{\judgeprop{\Theta}{\phi}{}} &: \comprehend{\delta}{|- \delta : \overline{\Theta}} \to \Set \\
    \sem{\delta}{t = t'}
      &=
      \begin{cases}
        \{\bullet\} &\quad\text{if } \sem{\delta}{t} = \sem{\delta}{t'} \\
        \emptyset &\quad\text{else}
      \end{cases}
    \\
    \sem{\delta}{t \leq t'}
      &=
      \begin{cases}
        \{\bullet\} &\quad\text{if } \sem{\delta}{t} \leq \sem{\delta}{t'} \\
        \emptyset &\quad\text{else}
      \end{cases}
    \\
    \sem{\delta}{\phi_1 \land \phi_2}
      &= \sem{\delta}{\phi_1} \cap \sem{\delta}{\phi_2}
    \\
    \sem{\delta}{\phi_1 \lor \phi_2}
      &= \sem{\delta}{\phi_1} \cup \sem{\delta}{\phi_2}
    \\
    \sem{\delta}{\neg\phi}
      &= \{\bullet\} \setminus \sem{\delta}{\phi}
    \\
    \sem{\delta}{\True}
      &= \{\bullet\}
    \\
    \sem{\delta}{\False}
      &= \emptyset
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
    %
  \end{align*}
  
  \caption{Denotational semantics of well-formed indexes and propositions}
  \label{fig:denotation-ix-prop}
\end{figure}

\begin{figure}[htbp]
  \judgbox{
    \judgeentail{\Theta}{\phi}
  }
  {
    Under $\Theta$, assertion or proposition $\phi$ is true
  }
  \begin{mathpar}
    \Infer{\PropTrue}
    {
      \text{for all }\delta\text{, if }|- \delta : \Theta\text{ then }
      \sem{\delta}{\phi} = \{\bullet\}
    }
    {\judgeentail{\Theta}{\phi}}
  \end{mathpar}

  \caption{Propositional truth}
  \label{fig:prop-truth}
\end{figure}


\begin{figure}[htbp]
  \centering
  
  %
  \begin{align*}
    \mu &: (\Set \to \Set) \to \Set \\
    \mu F &= \bigcup_{k=0}^{\infty} F^k \emptyset
    &\\[1em]
    \fold{}{}
        &:
          \prod_{F \in \Set \Rightarrow \Set}
          (F X \to X) \to \mu F \to X
          &\\
    \fold{F}{\alpha}
        &= \alpha \circ \left( \fmap{F}{(\fold{F}{\alpha}}) \right) \circ \mathrm{out}
    &\\[1em]
    \sem{}{\judgetp{\Theta}{A}{\Xi}} &: \comprehend{\delta}{|- \delta : \Theta} \to \Set \\
    \sem{\delta}{1}
        &=
        \{ \bullet \}
    &\\
    \sem{\delta}{P_1 \times P_2}
        &=
        \sem{\delta}{P_1} \times \sem{\delta}{P_2}
    &\\
    \sem{\delta}{0}
        &=
        \emptyset
    &\\
    \sem{\delta}{P_1 + P_2}
        &=
        \sem{\delta}{P_1} \uplus \sem{\delta}{P_2}
    &\\
    \sem{\delta}{ \comprehend{\nu : \mu F}{\Fold{F}{\alpha}\;\nu =_\tau t} }
        &=
        \comprehend{ d \in \mu\sem{\delta}{F} }
          { (\fold{\sem{\delta}{F}}{\sem{\delta}{\alpha}})\;d = \sem{\delta}{t} }
    &\\
    \sem{\delta}{
        \extype{a : \tau}{P}
        }
        &=
        \sum_{d \in \sem{}{\tau}} \sem{(\delta, d/a)}{P}
        %
    &\\
    \sem{\delta}{
        P \andty \phi
        }
        &=
        \sem{\delta}{P} \times  \sem{\delta}{\phi}
        %
        %
        %
        %
    &\\
    \sem{\delta}{
        \downshift{N}
        }
        &=
        \sem{\delta}{N}
    &\\
    \sem{\delta}{
        \alltype{a:\tau}{N}
        }
        &=
        %
        %
        \bigcap_{d \in \sem{}{\tau}} \sem{(\delta, d/a)}{N}
    &\\
    \sem{\delta}{
        P \to N
        }
        &=
        {\sem{\delta}{P}} \Rightarrow \sem{\delta}{N}
    &\\
    \sem{\delta}{
        \phi \implies N
        }
        &=
        {\sem{\delta}{\phi}} \Rightarrow \sem{\delta}{N}
    &\\
    \sem{\delta}{
        \upshift{P}
        }
        &=
        \sem{\delta}{P}
    &\\
    \sem{\delta}{
      \inferrule
      {
      \judgetp{\Theta}{A}{\Xi'}
      \\
      \Xi' \supseteq \Xi
      }
      {\judgetp{\Theta}{A}{\Xi}}
    } &= \sem{\delta}{\judgetp{\Theta}{A}{\Xi'}}
  \end{align*} 
  %
  
  \caption{Denotational semantics of well-formed types}
  \label{fig:denotation-types1}
\end{figure}

\begin{figure}[htbp]
  \centering
  
  %
  \begin{flalign*}
   \sem{}{\judgefunctor{\Theta}{\mathcal{F}}{\Xi}}
       &:
       \comprehend{\delta}{|- \delta : \Theta} \to \Set \to \Set
   &\\
   \sem{\delta}{F_1 \oplus F_2}
       &=
       X \mapsto \sem{\delta}{F_1} X \uplus \sem{\delta}{F_2} X
   &\\
   \sem{\delta}{I}
       &=
       X \mapsto \{ \bullet \}
   &\\
   \sem{\delta}{B \otimes \Ptype} 
       &=
       X \mapsto \sem{\delta}{B} X \times \sem{\delta}{\Ptype} X
   &\\
   \sem{\delta}{\Const{P}} 
       &=
       X \mapsto \sem{\delta}{P}
   &\\
   \sem{\delta}{\Id}
       &=
       X \mapsto X
   &\\
   \sem{\delta}{
     \inferrule
     {
       \judgefunctor{\Theta}{\mathcal{F}}{\Xi'}
       \\
       \Xi' \supseteq \Xi
     }
     {\judgefunctor{\Theta}{\mathcal{F}}{\Xi}}
   } &= \sem{\delta}{\judgefunctor{\Theta}{\mathcal{F}}{\Xi'}}
    &\\[2em]
    %
    %
    %
    %
    \sem{}{\judgealgebra{\Theta}{\alpha}{F}{\tau}}
        &: \prod_{\delta \in \comprehend{\delta}{|- \delta : \Theta}} \sem{\delta}{F}\sem{}{\tau} \to \sem{}{\tau}\\
    \sem{\delta}
      {\judgealgebra{\Theta}{\alpha}{(F_1 \oplus F_2)}{\tau}}
        &:
        \sem{\delta}{F_1 \oplus F_2}\big(\sem{}{\tau}\big)
            \to \sem{}{\tau}\\
    \sem{\delta}
      {\judgealgebra{\Theta}{\alpha}{(F_1 \oplus F_2)}{\tau}}
        d
        &=
        %
            \begin{cases}
              \sem{\delta}
                {\judgealgebra{\Theta}{\alpha_1}{F_1}{\tau}} d'
                  & \text{if }d = (1, d')\\
              \sem{\delta}
                {\judgealgebra{\Theta}{\alpha_2}{F_2}{\tau}} d'
                  & \text{if }d = (2, d')
              \end{cases}\\
        &\text{where }\composeinj{1}{\alpha}{\alpha_1}
        \text{ and }  \composeinj{2}{\alpha}{\alpha_1}
    &\\[0.5em]
    \sem{\delta}{\judgealgebra{\Theta}{\clause{\unitexp}{t}}{I}{\tau}}
        &=
        \bullet \mapsto \sem{\delta}{t}
    &\\[0.5em]
    %
    \sem{\delta}{\Theta |- \clause{(a, q)}{t} : %
                   \clause{(\Id \otimes \hat{P})(\tau)}{\tau}}
    %
        &:
        \sem{}{\tau} \times \big(\sem{\delta}{\hat{P}}(\sem{}{\tau})\big)
            \to \sem{}{\tau}
    &\\
    %
    \sem{\delta}{\Theta |- \clause{(a, q)}{t} : %
                   \clause{(\Id \otimes \hat{P})(\tau)}{\tau}}
        (d_1, d_2)
    %
        &=
        %
          \sem{(\delta, d_1/a)}{\Theta, a : \tau |- \clause{q}{t} :
                        \clause{\hat{P}(\tau)}{\tau}}
            d_2
    &\\[1.5em]
    %
    \sem{\delta}{\Theta |- \clause{(\wild, q)}{t} :%
    \clause{(\Const{Q} \otimes \hat{P})(\tau)}{\tau}}
    %
        &:
        %
        %
        \sem{\delta}{Q} \times \left(\sem{\delta}{\hat{P}}(\sem{}{\tau})\right)
            \to \sem{}{\tau}
    &\\
    %
    \sem{\delta}{\Theta |- \clause{(\wild, q)}{t} :%
                  \clause{(\Const{Q} \otimes \hat{P})(\tau)}{\tau}}
    %
        &=
        (\wild, d) \mapsto
        \sem{\delta}{\Theta |- \clause{q}{t} :
                       \clause{\hat{P}(\tau)}{\tau}} d
    &\\[0.5em]
    %
    \sem{\delta}{\Theta |- \clause{(\pack{a}{\bap}, q)}{t} : %
                 \clause{(\Const{\extype{a:\tau}{Q}} \otimes
                           \hat{P})(\tau)}{\tau}}
    %
        &:
        %
        %
        %
        %
        \left( \sum_{d\in\sem{}{\tau}} \sem{(\delta,d/a)}{Q} \right)
            \times \left( \sem{\delta}{\hat{P}}(\sem{}{\tau}) \right)
          \to \sem{}{\tau}
    &\\
    %
    \sem{\delta}{\Theta |- \clause{(\pack{a}{\bap}, q)}{t} :%
      \clause{(\Const{\extype{a:\tau}{Q}} \otimes \hat{P})(\tau)}{\tau}}
    %
        &=
        ((d, d'), d'') \mapsto \\
        &\sem{(\delta,d/a)}
            {\judgealgebra{\Theta,a:\tau}{\clause{(\bap, q)}{t}}
               {(\Const{Q} \otimes \hat{P})}{\tau}}
          (d', d'')
  \end{flalign*} 
  %
  
  \caption{Denotational semantics of well-formed functors and algebras}
  \label{fig:denotation-types2}
\end{figure}

\begin{figure}[htbp]
  \begin{flalign*}
    &\sem{}{\judgesub[\pm]{\Theta}{A}{B}} : \prod_{\delta \in \comprehend{\delta}{|- \delta : \Theta}} \sem{\delta}{A} \to \sem{\delta}{B} &\\
    &\sem{\delta}{\judgesub[+]{\Theta}{0}{0}}
      = \text{empty function} &\\
    &\sem{\delta}{\judgesub[+]{\Theta}{1}{1}}
      = \bullet \mapsto \bullet &\\
    &\sem{\delta}{\judgesub[+]{\Theta}{P_1 \times P_2}{Q_1 \times Q_2}}
      = (d_1, d_2) \mapsto \left( \sem{\delta}{\judgesub[+]{\Theta}{P_1}{Q_1}} d_1
        , \sem{\delta}{\judgesub[+]{\Theta}{P_2}{Q_2}} d_2 \right) &\\
    &\sem{\delta}{\judgesub[+]{\Theta}{P_1 + P_2}{Q_1 + Q_2}}
      = \begin{cases}
          (1, d) \mapsto (1, \sem{\delta}{\judgesub[+]{\Theta}{P_1}{Q_1}} d) \\
          (2, d) \mapsto (2, \sem{\delta}{\judgesub[+]{\Theta}{P_2}{Q_2}} d)
        \end{cases} &\\
    &\sem{\delta}{\judgesub[+]{\Theta}{P \land \phi}{Q}}
      = \begin{cases}
          (d,\bullet) \mapsto \sem{\delta}{\judgesub[+]{\Theta, \phi}{P}{Q}} d
              & \text{if }\sem{\delta}{\phi} = \{\bullet\} \\
          \text{empty function}
              & \text{else}
        \end{cases} &\\
    &\sem{\delta}{\judgesub[+]{\Theta}{\extype{a:\tau}{P}}{Q}}
      = (d, d') \mapsto \sem{\delta,d/a}{\judgesub[+]{\Theta, a:\tau}{P}{Q}} d' &\\
    &\sem{\delta}{
      \inferrule
      {\judgesub[+]{\Theta}{P}{Q} \\ \judgeentail{\Theta}{\phi} }
      {\judgesub[+]{\Theta}{P}{Q \land \phi} }
    } = d \mapsto (\sem{\delta}{\judgesub[+]{\Theta}{P}{Q}} d, \bullet) &\\
    &\sem{\delta}{
      \inferrule
      { 
        \judgesub[+]{\Theta}{P}{[t/a]Q} 
        \\
        \judgeterm{\Theta}{t}{\tau} 
      }
      {\judgesub[+]{\Theta}{P}{\extype{a:\tau}{Q}} }
    } = d \mapsto (\sem{\delta}{t}
                  , \sem{\delta}{\judgesub[+]{\Theta}{P}{[t/a]Q}} d) &\\
    &\sem{\delta}
       {\judgesub[+]{\Theta}
            {\comprehend{\nu:\mu F}{\Fold{F}{\alpha}\,\nu =_\tau t}}
            {\comprehend{\nu:\mu F}{\Fold{F}{\alpha}\,\nu =_\tau t'}}}
      = \id_{\mu\sem{\delta}{F}} &\\
    &\sem{\delta}{\judgesub[+]{\Theta}{\downshift{N}}{\downshift{M}}}
      = \sem{\delta}{\judgesub[-]{\Theta}{N}{M}} &\\
    &\sem{\delta}{\judgesub[-]{\Theta}{\upshift{P}}{\upshift{Q}}}
      = \sem{\delta}{\judgesub[+]{\Theta}{P}{Q}} &\\
    &\sem{\delta}{\judgesub[-]{\Theta}{N}{\phi \implies M}}
      = \begin{cases}
          d \mapsto (\bullet \mapsto
                       \sem{\delta}{\judgesub[-]{\Theta,\phi}{N}{M}} d)
            & \text{if }\sem{\delta}{\phi} = \{\bullet\} \\
          d \mapsto \text{empty function}
            & \text{else}
        \end{cases} &\\
    &\sem{\delta}{\judgesub[-]{\Theta}{N}{\alltype{a:\tau}{M}}}
      = d \mapsto (d' \mapsto \sem{\delta,d'/a}
                                  {\judgesub[-]{\Theta,a:\tau}{N}{M}} d) &\\
    &\sem{\delta}{
      \inferrule
      {\judgesub[-]{\Theta}{N}{M} \\ \judgeentail{\Theta}{\phi} }
      {\judgesub[-]{\Theta}{\phi \implies N}{M} }
    } = f \mapsto \sem{\delta}{\judgesub[-]{\Theta}{N}{M}} f(\bullet) &\\
    &\sem{\delta}{
      \inferrule
      {
        \judgesub[-]{\Theta}{[t/a]N}{M} 
        \\ 
        \judgeterm{\Theta}{t}{\tau} 
      }
      {\judgesub[-]{\Theta}{\alltype{a:\tau}{N}}{M} }
    } = f \mapsto \sem{\delta}{\judgesub[-]{\Theta}{[t/a]N}{M}}
                     f(\sem{\delta}{t}) &\\
    &\sem{\delta}{\judgesub[-]{\Theta}{P \to N}{Q \to M}}
      = f \mapsto \sem{\delta}{\judgesub[-]{\Theta}{N}{M}}
                    \circ f \circ \sem{\delta}{\judgesub[+]{\Theta}{Q}{P}} &
  \end{flalign*}

  \caption{Denotational semantics of subtyping}
  \label{fig:denotation-subtyping}
\end{figure}

\begin{figure}[htbp]
  \begin{flalign*}
    &\sem{}{\judgesynhead{\Theta}{\Gamma}{h}{P}} : \prod_{\delta\in\comprehend{\delta}{|- \delta : \Theta; \Gamma}} \sem{\delta}{P} &\\
    &\sem{\delta}{\judgesynhead{\Theta}{\Gamma}{x}{P}}
      = \delta(x) &\\
    &\sem{\delta}{\judgesynhead{\Theta}{\Gamma}{\annoexp{v}{P}}{P}}
      = \sem{\delta}{\judgechkval{\Theta}{\Gamma}{v}{P}}
    &\\[2em]
    &\sem{}{\judgesynexp{\Theta}{\Gamma}{\be}{N}} : \prod_{\delta\in\comprehend{\delta}{|- \delta : \Theta; \Gamma}} \sem{\delta}{N} &\\
    &\sem{\delta}{
      \inferrule
      {
        \judgesynhead{\Theta}{\Gamma}{h}{Q}
        \\
        \judgeleadsto{\Theta}{Q}{\downshift{N}}{\Phi}
        \\
        \judgespine{\Theta}{\Gamma}{s}{N}{\upshift{P}} }
      { \judgesynexp{\Theta}{\Gamma}{h(s)}{\upshift{P}} }
    } &\\
      &= \sem{\delta}{\judgespine{\Theta}{\Gamma}{s}{N}{\upshift{P}}}
         \left(
           \sem{\delta}{\judgeleadsto{\Theta}{Q}{\downshift{N}}{\Phi}}
           \sem{\delta}{\judgesynhead{\Theta}{\Gamma}{h}{Q}}
         \right) &\\
         &\text{where }
         \sem{\delta}{\judgeleadsto{\Theta}{Q}{\downshift{N}}{\Phi}} 
         : \sem{\delta}{Q} \to \sem{\delta}{\downshift{N}}
         = (d, \underbrace{\bullet, \dots, \bullet}_{|\Phi|}) \mapsto d &\\
    &\sem{\delta}{\judgesynexp{\Theta}{\Gamma}{\annoexp{e}{\upshift{P}}}
                     {\upshift{P}}}
      = \sem{\delta}{\judgechkexp{\Theta}{\Gamma}{e}{\upshift{P}}}
  \end{flalign*}

  \caption{Denotational semantics of (derivations of)
    head $h$ and bound expression $\be$ judgements}
  \label{fig:denotation-head-bound}
\end{figure}


\begin{figure}[htbp]
  \begin{flalign*}
    &\sem{}{\judgechkval{\Theta}{\Gamma}{v}{P}} : \prod_{\delta\in\comprehend{\delta}{|- \delta : \Theta; \Gamma}} \sem{\delta}{P} &\\
    &\sem{\delta}{
      \inferrule
      { (x:Q) \in \Gamma \\ \judgesub[+]{\Theta}{Q}{P} }
      { \judgechkval{\Theta}{\Gamma}{x}{P} }
    } = \sem{\delta}{\judgesub[+]{\Theta}{Q}{P}} \delta(x) &\\
    &\sem{\delta}{\judgechkval{\Theta}{\Gamma}{\unit}{1}}
      = \bullet &\\
    &\sem{\delta}{\judgechkval{\Theta}{\Gamma}{\pair{v_1}{v_2}}{P_1 \times P_2}}
      = ( \sem{\delta}{\judgechkval{\Theta}{\Gamma}{v_1}{P_1}}
         , \sem{\delta}{\judgechkval{\Theta}{\Gamma}{v_2}{P_2}}
         ) &\\
    &\sem{\delta}{\judgechkval{\Theta}{\Gamma}{\inj{k}{v}}{P_1 + P_2}}
      = (k, \sem{\delta}{\judgechkval{\Theta}{\Gamma}{v}{P_k}}) &\\
    &\sem{\delta}{
      \inferrule
      {
        \judgechkval{\Theta}{\Gamma}{v}{[t/a]P}
        \\
        \Intro{v} 
        \\
        \judgeterm{\Theta}{t}{\tau}
      }
      { \judgechkval{\Theta}{\Gamma}{v}{(\extype{a:\tau} P)} }
    } = ( \sem{\delta}{t}
         , \sem{\delta}{\judgechkval{\Theta}{\Gamma}{v}{[t/a]P}}
         ) &\\
    &\sem{\delta}{
      \inferrule
      {
        \judgechkval{\Theta}{\Gamma}{v}{P}
        \\
        \Intro{v}
        \\
        \judgeentail{\Theta}{\phi}
      }
      { \judgechkval{\Theta}{\Gamma}{v}{P \land \phi} }
    } = ( \sem{\delta}{\judgechkval{\Theta}{\Gamma}{v}{P}}
        , \bullet
        ) &\\
    &\sem{\delta}{\judgechkval{\Theta}{\Gamma}{\roll{v}}
           {\comprehend{\nu:\mu F}{\Fold{F}{\alpha}\;\nu =_\tau t}}} &\\
         &= \mathrm{into} \left(
           \sem{\delta}{
             \judgeunroll{\Theta}
               {\nu:F[\mu F]}{\alpha}{F\;\Fold{F}{\alpha}\;\nu}{t}{P}{\tau} }^{-1}
        \sem{\delta}{\judgechkval{\Theta}{\Gamma}{v}{P}} \right) &\\
    &\sem{\delta}{\judgechkval{\Theta}{\Gamma}{\thunk{e}}{\downshift{N}}}
      = {\sem{\delta}{\judgechkexp{\Theta}{\Gamma}{e}{N}}}
    &\\[2em]
    &\sem{}{\judgechkexp{\Theta}{\Gamma}{e}{N}} : \prod_{\delta\in\comprehend{\delta}{|- \delta : \Theta; \Gamma}} \sem{\delta}{N} &\\
    &\sem{\delta}{\judgechkexp{\Theta}{\Gamma}{\Return{v}}{\upshift{P}}}
      = \sem{\delta}{\judgechkval{\Theta}{\Gamma}{v}{P}} &\\
    &\sem{\delta}{
      \inferrule
            { \judgesynexp{\Theta}{\Gamma}{\be}{\upshift{P}} \\
              \judgechkexp{\Theta}{\Gamma, x:P}{e}{N} }
            { \judgechkexp{\Theta}{\Gamma}{\Let{x}{\be}{e}}{N} }
    } = \sem{(\delta, 
                  \sem{\delta}{\judgesynexp{\Theta}{\Gamma}{\be}{\upshift{P}}}/x)}
             {\judgechkexp{\Theta}{\Gamma, x:P}{e}{N}} &\\
    &\sem{\delta}{\judgechkexp{\Theta}{\Gamma}{\fun{x}{e}}{P \to N}}
      = d \mapsto \sem{(\delta, d/x)}{\judgechkexp{\Theta}{\Gamma, x:P}{e}{N}} &\\
    &\sem{\delta}{\judgechkexp{\Theta}{\Gamma}{\rec{f}{e}}{N}}
      = \text{the element }d \in \sem{\delta}{N}\text{ such that }
        d = \sem{\delta,d/f}{\judgechkexp{\Theta}{\Gamma, f:\downshift{N}}{e}{N}} &\\
    &\sem{\delta}
        {\judgechkexp{\Theta}{\Gamma}{\match{h}{\clauses{\pa}{e}{i}{I}}}{N}}
      = \sem{\delta}{\judgechkmatch{\Theta}{\Gamma}{P}{\clauses{\pa}{e}{i}{I}}{N}}
          \sem{\delta}{\judgesynhead{\Theta}{\Gamma}{h}{P}} &\\
    &\sem{\delta}{\judgechkexp{\Theta}{\Gamma}{e}{\phi \implies N}}
      = \bullet \mapsto \sem{\delta}{\judgechkexp{\Theta, \phi}{\Gamma}{e}{N}} &\\
    &\sem{\delta}{\judgechkexp{\Theta}{\Gamma}{e}{(\alltype{a:\tau} N)}}
      = d \mapsto \sem{\delta,d/a}{\judgechkexp{\Theta, a:\tau}{\Gamma}{e}{N}}
  \end{flalign*}

  \caption{Denotational semantics of (derivations of)
    value $v$ and expression $e$ judgements}
  \label{fig:denotation-val-exp}
\end{figure}

\begin{figure}[htbp]
  \begin{flalign*}
    &\sem{}{\judgechkmatch{\Theta}{\Gamma}{P}{\clauses{\pa}{e}{i}{I}}{N}} : \prod_{\delta\in\comprehend{\delta}{|- \delta : \Theta; \Gamma}} \sem{\delta}{P} \to \sem{\delta}{N} \\
    &\sem{\delta}{\judgechkmatch{\Theta}{\Gamma}{1}{\setof{\clause{\unit}{e}}}{N}}
      = \bullet \mapsto \sem{\delta}{\judgechkexp{\Theta}{\Gamma}{e}{N}} \\
    &\sem{\delta}{\judgechkmatch{\Theta}{\Gamma}{P_1 \times P_2}
        {\setof{\clause{\pair{x_1}{x_2}}{e}}}{N}}
      = (d_1, d_2) \mapsto \sem{(\delta,d_2/x_2,d_1/x_1)}
                             {\judgechkexp{\Theta}{\Gamma, x_2:P_2, x_1:P_1}{e}{N}} \\
    &\sem{\delta}{\judgechkmatch{\Theta}{\Gamma}{P_1 + P_2}
                  {\setof{ \clause{\inl{x_1}}{e_1} \bnfalt \clause{\inr{x_2}}{e_2}}}{N}}
      = \begin{cases}
          (1, d_1) \mapsto
             \sem{\delta,d_1/x_1}{\judgechkexp{\Theta}{\Gamma, x_1:P_1}{e_1}{N}} \\
          (2, d_2) \mapsto
             \sem{\delta,d_2/x_2}{\judgechkexp{\Theta}{\Gamma, x_2:P_2}{e_2}{N}} 
        \end{cases} \\
    &\sem{\delta}{\judgechkmatch{\Theta}{\Gamma}{0}{\setof{}}{N}}
       = \text{the empty function from }\emptyset\text{ to }\sem{\delta}{N} \\
    &\sem{\delta}{\judgechkmatch{\Theta}{\Gamma}
                     {\comprehend{\nu:\mu F}{\Fold{F}{\alpha}\;\nu =_\tau t}}
                     {\setof{\clause{\roll{x}}{e}}}{N}} \\
      &= d \mapsto \text{let }d' = 
         \sem{\delta}
           {
             \judgeunroll{\Theta}{\nu:F[\mu F]}
                {\alpha}{F\;\Fold{F}{\alpha}\;\nu}{t}{P}{\tau}
           }
         (\mathrm{out}\;d)
         \text{ in }\sem{\delta,d'/x}{\judgechkexp{\Theta}{\Gamma, x:P}{e}{N}}
         \\
    &\sem{\delta}
       {\judgechkmatch{\Theta}{\Gamma}{\extype{a:\tau}{P}}{\clauses{\pa}{e}{i}{I}}{N}}
       = (d, d') \mapsto
            \sem{\delta,d/a}
              {\judgechkmatch{\Theta,a:\tau}{\Gamma}{P}{\clauses{\pa}{e}{i}{I}}{N}} d' \\
    &\sem{\delta}
         {\judgechkmatch{\Theta}{\Gamma}{P \land \phi}{\clauses{\pa}{e}{i}{I}}{N}}
         = (d, \bullet) \mapsto \sem{\delta}
                                {\judgechkmatch{\Theta,\phi}{\Gamma}
                                   {P}{\clauses{\pa}{e}{i}{I}}{N}} d
    \\[2em]
    &\sem{}{\judgespine{\Theta}{\Gamma}{s}{N}{M}} : \prod_{\delta\in\comprehend{\delta}{|- \delta : \Theta; \Gamma}} \sem{\delta}{N} \to \sem{\delta}{M} \\
    &\sem{\delta}{
      \inferrule
      {
        \judgeterm{\Theta}{t}{\tau}
        \\
        \judgespine{\Theta}{\Gamma}{s}{[t/a]N}{\upshift{P}}
      }
      {\judgespine{\Theta}{\Gamma}{s}{(\alltype{a:\tau}{N})}{\upshift{P}}}
    } = f \mapsto 
            \sem{\delta}{\judgespine{\Theta}{\Gamma}{s}{[t/a]N}{\upshift{P}}}
              \left( f \sem{\delta}{t} \right)\\
    &\sem{\delta}{
      \inferrule
      {\judgeentail{\Theta}{\phi} \\ \judgespine{\Theta}{\Gamma}{s}{N}{\upshift{P}}}
      {\judgespine{\Theta}{\Gamma}{s}{(\phi \implies N)}{\upshift{P}}}
    } = f \mapsto
             \sem{\delta}
               {\judgespine{\Theta}{\Gamma}{s}{N}{\upshift{P}}}
                    \left( f(\bullet) \right)\\
    &\sem{\delta}{\judgespine{\Theta}{\Gamma}{v,s}{Q \to N}{\upshift{P}}}
      = f \mapsto \sem{\delta}{\judgespine{\Theta}{\Gamma}{s}{N}{\upshift{P}}}
             \left(f\sem{\delta}{\judgechkval{\Theta}{\Gamma}{v}{Q}}\right) \\
    &\sem{\delta}{\judgespine{\Theta}{\Gamma}{\cdot}{\upshift{P}}{\upshift{P}}}
       = \id_{\sem{\delta}{\upshift{P}}} 
  \end{flalign*}

  \caption{Denotational semantics of (derivations of) matching and spine judgements}
  \label{fig:denotation-match-spine}
\end{figure}

\begin{figure}[htbp]
  \raggedright
  %
  For \DeclUnrollSum:\\
  %
  $
    \sem{\delta}{\judgeunroll{\Theta}{\nu:(G \oplus H)[\mu F]}{\beta}
      {(G \oplus H)\;\Fold{F}{\alpha}\;\nu}{t}{P + Q}{\tau}}
  $
  \begin{align*}
    \quad :& \comprehend
    {d\in\sem{\delta}{G}(\mu\sem{\delta}{F})\uplus\sem{\delta}{H}(\mu\sem{\delta}{F})}
    {
      \sem{\delta}{\beta}
      (\sem{\delta}{G \oplus H}(\fold{\sem{\delta}{F}}{\sem{\delta}{\alpha}}))\;d
      =
      \sem{\delta}{t}
    } \\
    \quad \to& \sem{\delta}{P+Q} \\
    \quad =&\; d \\
    \quad \mapsto& \begin{cases}
      \minj{1} (\sem{\delta}{\judgeunroll{\Theta}{\nu:G[\mu F]}
        {\beta_1}{G\;\Fold{F}{\alpha}\;\nu}{t}{P}{\tau}} d')
      & \text{if }d=(1,d') \\
      \minj{2} (\sem{\delta}{\judgeunroll{\Theta}{\nu:H[\mu F]}
        {\beta_2}{H\;\Fold{F}{\alpha}\;\nu}{t}{Q}{\tau}} d')
      & \text{if }d=(2,d')
      \end{cases}
  \end{align*}
  $
  \sem{\delta}{\judgeunroll{\Theta}{\nu:(G \oplus H)[\mu F]}{\beta}
    {(G \oplus H)\;\Fold{F}{\alpha}\;\nu}{t}{P + Q}{\tau}}^{-1}
  $
  \begin{align*}
    \quad =&\;d \\
    \quad \mapsto& \begin{cases}
      \minj{1} (\sem{\delta}{\judgeunroll{\Theta}{\nu:G[\mu F]}
        {\beta_1}{G\;\Fold{F}{\alpha}\;\nu}{t}{P}{\tau}}^{-1} d')
      & \text{if }d=(1,d') \\
      \minj{2} (\sem{\delta}{\judgeunroll{\Theta}{\nu:H[\mu F]}
        {\beta_2}{H\;\Fold{F}{\alpha}\;\nu}{t}{Q}{\tau}}^{-1} d')
      & \text{if }d=(2,d')
    \end{cases}
  \end{align*}
  \\
  %
  For \DeclUnrollId:\\
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
  $
  \sem{\delta}{
    \judgeunroll*{\Theta}{\nu : (\Id\otimes\hat{P})[\mu F]}
    {(\clause{(a,q)}{t'})}
    {(\Id\otimes\hat{P})\;\Fold{F}{\alpha}\;\nu}{t}
    {\extype{a:\tau}
      {\comprehend{\nu:\mu F}{ \Fold{F}{\alpha}\,{\nu} =_\tau a } \times Q}}
    {\tau}
  }
  $
  \begin{align*}
    \quad :&\;
      \big\{
      (d_1,d_2)\in\mu\sem{\delta}{F}\times\sem{\delta}{\hat{P}}\mu\sem{\delta}{F}
      \;\big|\;
               \sem{\delta}{\clause{(a,q)}{t'}}
               \left(
               (\fold{\sem{\delta}{F}}{\sem{\delta}{\alpha}})\;d_1
               ,
               \sem{\delta}{\hat{P}}
               (\fold{\sem{\delta}{F}}{\sem{\delta}{\alpha}})\;d_2
               \right)
               = \sem{\delta}{t}
               \big\} \\
    \quad \to& \sum_{d \in \sem{}{\tau}}
             \comprehend{d'\in\mu\sem{\delta}{F}}
             {(\fold{\sem{\delta}{F}}{\sem{\delta}{\alpha}})\;d' = d}
             \times \sem{\delta,d/a}{Q} \\
    \quad =&\;(d_1,d_2) \\
    \quad \mapsto&\;
                   \left( d,
                   \left(d_1, \sem{\delta,d/a}{\judgeunroll{\Theta, a:\tau}{\nu:\hat{P}[\mu F]}
                   {(\clause{q}{t'})}{\hat{P}\;\Fold{F}{\alpha}\;\nu}
                   {t}{Q}{\tau}} d_2
                   \right)
                   \right)\\
    \quad &~~~~\text{where }d=(\fold{\sem{\delta}{F}}{\sem{\delta}{\alpha}})\;d_1
  \end{align*}
  $
  \sem{\delta}{
    \judgeunroll*{\Theta}{\nu : (\Id\otimes\hat{P})[\mu F]}
    {(\clause{(a,q)}{t'})}
    {(\Id\otimes\hat{P})\;\Fold{F}{\alpha}\;\nu}{t}
    {\extype{a:\tau}
      {\comprehend{\nu:\mu F}{ \Fold{F}{\alpha}\,{\nu} =_\tau a } \times Q}}
    {\tau}
  }^{-1}
  $
  \begin{align*}
    \quad =&\;(d,(d_1,d_2)) \\
    \quad \mapsto& 
                   \left(d_1, \sem{\delta,d/a}{\judgeunroll{\Theta, a:\tau}{\nu:\hat{P}[\mu F]}
                   {(\clause{q}{t'})}{\hat{P}\;\Fold{F}{\alpha}\;\nu}
                   {t}{Q}{\tau}}^{-1} d_2\right)
  \end{align*}
  
  \caption{Denotation semantics of (derivations of) refinement type unrolling judgements
    (part 1)}
  \label{fig:denotation-unroll1}
\end{figure}

\begin{figure}[htbp]
  \raggedright
  %
  For \DeclUnrollConstEx:\\
  %
  $
  \sem{\delta}{
    \judgeunroll{\Theta}{\nu :(\Const{\extype{a:\tau}{Q}}\otimes\hat{P})[\mu F]}{(\clause{(\pack{a}{\bap}, q)}{t})}{(\Const{\extype{a:\tau}{Q}}\otimes\hat{P})\;\Fold{F}{\alpha}\;\nu}{t}{\extype{a:\tau}{Q'}}{\tau}
  }
  $
  \begin{align*}
    \quad :& \comprehend
               {((d,d'),d'')\in\left(\sum_{d\in\sem{}{\tau}}\sem{\delta,d/a}{Q}\right)\times\sem{\delta}{\hat{P}}(\mu\sem{\delta}{F})}
               {
               \sem{\delta}{\clause{(\bap,q)}{t'})}
               (d, \sem{\delta}{\hat{P}}
               (\fold{\sem{\delta}{F}}{\sem{\delta}{\alpha}})\;d')
               = \sem{\delta}{t}
               }\\
    \quad \to& \sum_{d\in\sem{}{\tau}}\sem{\delta,d/a}{Q'} \\
    \quad =&\; ((d, d'),d'') \\
    \quad \mapsto& \left(d, \sem{\delta,d/a}{\judgeunroll{\Theta,a:\tau}
                   {\nu:(\Const{Q}\otimes\hat{P})[\mu
                   F]}{(\clause{(\bap,q)}{t'})}{(\Const{Q}\otimes\hat{P})\;\Fold{F}{\alpha}\;\nu}{t}{Q'}{\tau}}
                   (d',d'')\right)
  \end{align*}
  $
  \sem{\delta}{
    \judgeunroll{\Theta}{\nu :(\Const{\extype{a:\tau}{Q}}\otimes\hat{P})[\mu F]}{(\clause{(\pack{a}{\bap}, q)}{t})}{(\Const{\extype{a:\tau}{Q}}\otimes\hat{P})\;\Fold{F}{\alpha}\;\nu}{t}{\extype{a:\tau}{Q'}}{\tau}
  }^{-1}
  $
  \begin{align*}
    \quad =&\; (d, d') \\
    \quad \mapsto&\;\text{let }(d_1,d_2) = 
                   \sem{\delta,d/a}{\judgeunroll{\Theta,a:\tau}
                   {\nu:(\Const{Q}\otimes\hat{P})[\mu
                   F]}{(\clause{(\bap,q)}{t'})}{(\Const{Q}\otimes\hat{P})\;\Fold{F}{\alpha}\;\nu}{t}{Q'}{\tau}}^{-1} d'\\
    \quad &\;\text{in }((d,d_1),d_2)
  \end{align*}
  %
  For \DeclUnrollConst:\\
  %
  $
  \sem{\delta}{
    \judgeunroll{\Theta}{\nu :(\Const{Q}\otimes\hat{P})[\mu F]}{(\clause{(\wild,q)}{t'})}{(\Const{Q}\otimes\hat{P})\;\Fold{F}{\alpha}\;\nu}{t}{Q \times Q'}{\tau}
  }
  $
  \begin{align*}
    \quad :& \comprehend
               {(d,d')\in\sem{\delta}{Q}\times\sem{\delta}{\hat{P}}(\mu\sem{\delta}{F})}
               {
               \sem{\delta}{\clause{(\wild,q)}{t'})}
               (d, \sem{\delta}{\hat{P}}
               (\fold{\sem{\delta}{F}}{\sem{\delta}{\alpha}})\;d')
               = \sem{\delta}{t}
               }\\
    \quad \to& \sem{\delta}{Q \times Q'} \\
    \quad =&\; (d, d') \\
    \quad \mapsto& \left(d, \sem{\delta}{\judgeunroll{\Theta}
                   {\nu:\hat{P}[\mu
                   F]}{(\clause{q}{t'})}{\hat{P}\;\Fold{F}{\alpha}\;\nu}{t}{Q'}{\tau}}
                   d'\right)
  \end{align*}
  $
  \sem{\delta}{
    \judgeunroll{\Theta}{\nu :(\Const{Q}\otimes\hat{P})[\mu F]}{(\clause{(\wild,q)}{t'})}{(\Const{Q}\otimes\hat{P})\;\Fold{F}{\alpha}\;\nu}{t}{Q \times Q'}{\tau}
  }^{-1}
  $
  \begin{align*}
    \quad =&\; (d, d') \\
    \quad \mapsto& \left(d, \sem{\delta}{\judgeunroll{\Theta}
                   {\nu:\hat{P}[\mu
                   F]}{(\clause{q}{t'})}{\hat{P}\;\Fold{F}{\alpha}\;\nu}{t}{Q'}{\tau}}^{-1}
                   d'\right)
  \end{align*}
  %
  For \DeclUnrollUnit:\\
  %
  $
  \sem{\delta}{\judgeunroll{\Theta}{\nu:I[\mu F]}{(\clause{\unitexp}{t'})}{I\;\Fold{F}{\alpha}\;\nu}{t}{1 \land (t = t')}{\tau}}
  $
  \begin{align*}
    \quad :& \comprehend{d \in \{\bullet\}}{\sem{\delta}{t'} = \sem{\delta}{t}} \\
    \quad \to&\; \{\bullet\}\times\sem{\delta}{t=t'} \\
    \quad =& \begin{cases}
      \bullet \mapsto
        (\bullet,\bullet) & \text{if } \sem{\delta}{t=t'} = \{\bullet\} \\
      \id_\emptyset  & \text{else}
      \end{cases}
  \end{align*}
  $
  \sem{\delta}{\judgeunroll{\Theta}{\nu:I[\mu F]}{(\clause{\unitexp}{t'})}{I\;\Fold{F}{\alpha}\;\nu}{t}{1 \land (t = t')}{\tau}}^{-1}
  $
  \[
  \quad = \begin{cases}
    (\bullet,\bullet)\mapsto\bullet & \text{if }\sem{\delta}{t=t'} = \{\bullet\} \\
    \id_\emptyset  & \text{else}
  \end{cases}
  \]
  
  \caption{Denotation semantics of (derivations of) refinement type unrolling judgements
    (part 2)}
  \label{fig:denotation-unroll2}
\end{figure}

%
%
%


==> fig-evar-unrolled-types.tex <==
\begin{figure}[htbp]
  \begin{grammar}
    $\ahat$-unrolled sum types  & 
    $\evarunrolltype{\ahat}{S}$ & \bnfas
    & $\evarunrolltype{\ahat}{P}
    \bnfalt \evarunrolltype{\ahat}{S} + \evarunrolltype{\ahat}{S}
    $
    \\
    $\ahat$-unrolled product types  & 
    $\evarunrolltype{\ahat}{P}$ & \bnfas
    & $1 \land \ahat = t
    \bnfalt \extype{a:\tau}{\evarunrolltype{\ahat}{P}}
    \bnfalt P \times \evarunrolltype{\ahat}{P}
    $
  \end{grammar}

  \caption{$\ahat$-unrolled types}
  \label{fig:evar-unrolled-types}
\end{figure}


%
%
%

